Poster: On the Feasibility of Training Neural Networks with Visibly Watermarked Dataset

As there are increasing needs of sharing data for machine learning, there is growing attention for the owners of the data to claim the ownership. Visible watermarking has been an effective way to claim the ownership of visual data, yet the visibly watermarked images are not regarded as a primary source for learning visual recognition models due to the lost visual information by in the watermark and the possibility of an attack to remove the watermarks. To make the watermarked images better suited for machine learning with less risk of removal, we propose DeepStamp, a watermarking framework that, given a watermarking image and a trained network for image classification, learns to synthesize a watermarked image that are human-perceptible, robust to removals, and able to be used as training images for classification with minimal accuracy loss. To achieve the goal, we employ the generative multi-adversarial network (GMAN). In experiments with CIFAR10, we show that the DeepStamp learn to transform a watermark to be embedded in each image and the watermarked images can be used to train networks.

==> sections/related.tex <==

\section{Related Work}
\label{sec:related}

%%%% Related work: saved for the Journal submission %%%%
% \subsection{Visible Watermarks}

% We focus our discussion on visible watermarks superimposed on images in the rest of our paper. Recent progress on digital watermarking techniques can be found in the survey papers, e.g.,~\cite{honsinger2002digital,potdar2005survey}. Braudaway et al.~\cite{braudaway1996protect} were the first to propose visible watermarks on digital images. They used adaptive, nonlinear pixel-domain technique to blend a watermark to an image to identify the ownership, which makes the watermark hard to remove and not to obscure the image details. This scheme has been extended invarious ways. Meng and Chang~\cite{meng1998embedding} applied the method to DCT domain and embedded watermarks to video streams. Kankanhalli and Ramakrishnan~\cite{kankanhalli1999adaptive} used statistic information of block DCT coefficients to determine the watermark embedding coefficients for each block. This technique is later extended to preserve the texture sensitivity in the human visual system to improve the perceptual quality of the images~\cite{mohanty2000dct}. Hu and Kwong~\cite{hu2001wavelet} proposed a visible watermarking method in a wavelet domain to tackle the visual discontinuities that can be occurred by DCT-based techniques. Despite the various techniques that improves the quality of watermarked images and makes the watermarks hard to remove, in practice, most stock content marketplaces use a standard additive watermarking method.

% Researchers, at the same time, have looked into various attacks that remove watermarks blended to images because they are important to claim the intellectual property (IP) of the images. Huang and Wu~\cite{huang2001inpainting} used typical image inpainting methods~\cite{bertalmio2000image} to fill the area covered by the watermark. Pei and Zeng~\cite{pei2006novel} proposed a novel attack that utilizes independent component analysis (ICA) to separate source images from watermarked and reference images. Dekel et al.~\cite{dekel2017effectiveness} demonstrated an attack that removes the watermarks by estimating the foreground, alpha matte, and background from the watermarked images. They also showed that random perturbations in the alpha matte can increase the robustness to this attack. 

% [SHHONG] videos are not in our interest: they used the inpainting from nearby frames
% Prior work also used the inpainting technique to remove the watermarks in video streams~\cite{wang2007automatic,yan2005automatic,dashti2015video}. Those attacks estimate the original image of the watermarked area from the nearby frames and removes the watermarks by substituting the watermarked area to the original corresponding component. However, in the stock photo markets, there is no reference images (e.g., nearby frames) where an attacker can estimate the original image of the watermarked area.


% % --- image perturbations: related to adversarial samples
% \subsection{Image Perturbations and Neural Networks}

% Recent work in adversarial examples has demonstrated that using the images with the perturbations hardly perceptible to humans can cause misclassifications of neural networks. Szegedy et al.~\cite{szegedy2013intriguing} was the first to find this property, and Goodfellow et al.~\cite{goodfellow6572explaining} showed that neural networks are vulnerable to adversarial samples because of their linear nature. They can synthesize such samples across architectures and training datasets. \cite{kurakin2016adversarial} demonstrated ...

% Adversarial samples are transferrable~\cite{papernot2016transferability}.

% Prior work has demonstrated that the perturbations on images invisible to human eyes can cause misclassifications of the images when they are fed to convolutional neural networks~\cite{goodfellow6572explaining,kurakin2016adversarial,liu2016delving,moosavi2016deepfool}. 

% what disadvantage can be incurred to achieve the robustness
% + what actually our technique can improve the robustness...
% [essential] cite the papers discussing the performance drops by using watermarked data...

% \cite{zhu2018hidden} demonstrated that, by jointly training deep neural networks, we can embed the specific information to images, not perceptible to human eyes.



% --- Generative networks
% \subsection{Generative Networks.}

% Generative adversarial networks~\cite{goodfellow2014generative} (GANs) and variational autoencoders~\cite{kingma2013auto} (VAEs) enable to estimate the generative models. GANs utilize an adversarial process; the generator (G) synthesizes the fake samples, and the discriminator (D) predicts whether a sample comes from the training data or from the generator. Once the training process reaches the equilibrium state where the D cannot identify if a sample is from G or not, the G has the ability to create samples under the training data distributions. On the other hand, VAEs learn the latent representations (or the embeddings) from inputs via encoding and decoding process; the encoder creates the embeddings of inputs, and the decoder synthesizes the outputs from them close to the inputs. After training, the decoder can generate the outputs from the given embeddings similar to the training data.

% Prior works have proposed various GANs and VAEs. Radford et al.~\cite{radford2015unsupervised} present deep convolutional generative adversarial networks (DCGANs) that enable to learn good representations of images. Chen et al.~\cite{chen2016infogan} propose InfoGAN that maximizes the mutual information between a small subset of the latent variables and the observation. Zhao et al.~\cite{zhao2016energy} present the energy-based generative adversarial network (EBGAN) that views the discriminator as an energy function. They substitute the D network in a GAN into VAE and achieve more stable behavior during training. Durugkar et al.~\cite{durugkar2016generative} propose the generative multi-adversarial network (GMAN) that utilizes multiple discriminators to obtain high-quality samples from the generator within the smaller number of iterations.

% Such capability of generative networks has been enabled various applications in the image synthesis domain. Ledig et al.~\cite{ledig2017photo} create the super-resolution images from the lower resolution images leveraging the SRGAN. \cite{pathak2016context, li2017generative} demonstrate that we can achieve image inpaintings by using the variational autoencoders. Zhu et al. and Isola et al.~\cite{CycleGAN2017, isola2017image} present an approach to translating an image between domains utilizing the GAN. Xian et al.~\cite{xian2017texturegan} synthesize images with the color stroke and texture patches. \cite{gadelha20173d} demonstrate that 3-D object images can be generated from 2-D images.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
